A new sampling indicator function for stable imaging of periodic scattering media

This paper is concerned with the inverse problem of determining the shape of penetrable periodic scatterers from scattered field data. We propose a sampling method with a novel indicator function for solving this inverse problem. This indicator functionl is very simple to implement and robust against noise in the data. The resolution and stability analysis of the indicator function is analyzed. Our numerical study shows that the proposed sampling method is more stable than the factorization method and more efficient than the direct or orthogonality sampling method in reconstructing periodic scatterers.

==> OSM periodic/mathmacros.tex <==
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}

%\renewcommand{\phi}{\phi}
\renewcommand{\d}{\mathrm{d}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\ol}{\overline}
\renewcommand{\i}{\mathrm{i}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\mur}{\mu_{\mathrm{r}}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\per}{\mathrm{per}}
\newcommand{\p}{\mathrm{p}}
\newcommand{\smooth}{\text{sm}}
\newcommand{\RR}{R}
\newcommand{\T}{\mathcal{T}}
\renewcommand{\sc}{\mathrm{sc}}
\newcommand{\inc}{\mathrm{inc}}


\DeclareMathOperator{\sign}{\mathrm{sign}}
\DeclareMathOperator{\Id}{\mathrm{Id}}


% \newtheorem{remark}[theorem]{Remark}

\renewcommand{\Re}{\mathrm{Re}\,}
\renewcommand{\Im}{\mathrm{Im}\,}
 \newcommand{\smalf}{\par\smallskip\noindent}
 \newcommand{\medlf}{\par\medskip\noindent}
 \newcommand{\biglf}{\par\bigskip\noindent}

\newcommand{\om}{\omega}
\newcommand{\eps}{\varepsilon}
\newcommand{\epsr}{\varepsilon_\mathrm{r}}
\newcommand{\epsi}{\epsilon}
\newcommand{\oD}{\overline{D}}
\newcommand{\oS}{\overline{S}}
\newcommand{\ov}{\overline}
\newcommand{\pD}{\partial D}
\newcommand{\cO}{{\cal O}}
\renewcommand{\H}{{\mathbf{H}}}
\newcommand{\vbH}{{\vec{\bm{H}}}}
\newcommand{\E}{{\mathbf{E}}}
\newcommand{\Ei}{{\mathbf{E}_\mathrm{in}}}
\newcommand{\Es}{{\mathbf{E}_\mathrm{sc}}}

\newcommand{\vbE}{{\vec{\bm{E}}}}
\newcommand{\vbJ}{{\vec{\bf J}}}
\newcommand{\vbA}{\mathcal{\bm{A}}}
\newcommand{\D}{{\mathbf{D}}}
\newcommand{\B}{{\mathbf{B}}}
\newcommand{\bRe}{{\bm{\mathcal{R}}^\epsilon}}
\newcommand{\bTe}{{\bm{\mathcal{T}}^\epsilon}}
\newcommand{\vbD}{{\vec{\bm{D}}}}
\newcommand{\curll}{{\vec{\nabla}\times}}
\newcommand{\divv}{{\vec{\nabla}\cdot}}
\renewcommand{\div}{\mathrm{div}}
\newcommand{\curl}{\mathrm{curl}\,}
\newcommand{\divtt}{{\nabla^\bot\cdot}}
\newcommand{\cN}{{\cal N}}
\newcommand{\cR}{{\cal R}}
\newcommand{\pa}{\partial}
\newcommand{\nal}{\nabla_{\alpha}}
\newcommand{\nalT}{\nabla_{\alpha,T}}
\newcommand{\naT}{\nabla_T}
\newcommand{\intO}{\int_{\Omega}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\f}{\mathbf{f}}
\renewcommand{\u}{\mathbf{u}}
\renewcommand{\v}{\mathbf{v}}

\newcommand{\bw}{\mathbf{w}}



%\newcommand{\vbz}{\vec{\bm{z}}}
%\newcommand{\vx}{\vbx}
%\newcommand{\bx}{\bm{x}}
%\newcommand{\vbn}{\vec{\bm{n}}}
%\newcommand{\vbut}{\vec{\bm{u}}^t}
%\newcommand{\vbui}{\vec{\bm{u}}^i}
%\newcommand{\vbuis}{\vec{\bm{u}}^{i(s')}}
%\newcommand{\vbu}{\vec{\bm{u}}}
%\newcommand{\vbg}{\vec{\bm{g}}}
%\newcommand{\vbf}{\vec{\bm{f}}}
%\newcommand{\vbw}{\vec{\bm{w}}}
%\newcommand{\vbv}{\vec{\bm{v}}}
%\newcommand{\vbphi}{\vec{\bm{\varphi}}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cm}{{\mathcal M}}
\newcommand{\lin}{\big<}
\newcommand{\rin}{\big>}
\newcommand{\bV}{\boldsymbol{\mathcal{V}}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bd}{{\bf d}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\icu}{{\mbox{\tiny curl}}}
\newcommand{\idiv}{{\mbox{\tiny div}}}

